SandCell: Sandboxing Rust Beyond Unsafe Code

Rust is a modern systems programming language that ensures memory safety by enforcing ownership and borrowing rules at compile time. While the unsafe keyword allows programmers to bypass these restrictions, it introduces significant risks. Various approaches for isolating unsafe code to protect safe Rust from vulnerabilities have been proposed, yet these methods provide only fixed isolation boundaries and do not accommodate expressive policies that require sandboxing both safe and unsafe code. This paper presents SandCell for flexible and lightweight isolation in Rust by leveraging existing syntactic boundaries. SandCell allows programmers to specify which components to sandbox with minimal annotation effort, enabling fine-grained control over isolation. The system also introduces novel techniques to minimize overhead when transferring data between sandboxes. Our evaluation demonstrates SandCell's effectiveness in preventing vulnerabilities across various Rust applications while maintaining reasonable performance overheads.

==> Makefile <==

ISPELLPAT = -ktexskip1 +cref,Cref,url,todo,presetkeys,newcommand,definecolor


all: main.pdf

main.pdf: *.tex 
	latexmk -shell-escape -pdflatex='pdflatex -file-line-error' -pdf main.tex


spelling: *.tex sections/*.tex
	for file in *.tex sections/*.tex; do \
          ispell -t ${ISPELLPAT} -b -d american -p ./paper.dict $$file; \
        done

clean:
	latexmk -C -pdflatex='pdflatex -file-line-error' -pdf main.tex
	rm -f main.pdf
	rm -f *.tex.bak

distclean: clean
	rm -f main.bbl


==> fig/dataflow-algo.tex <==
\begin{algorithm}[t]
\caption{Heap Objects on Boundaries.}\label{alg:dataflow}
\begin{algorithmic}
\Require Dataflow Grpah $G = (V, E)$.
\Require Set of places on boundaries $S$.
\Ensure  $S \subset V$.
\State $Q \gets \varnothing$ \Comment{An empty queue.}
\State $A \gets \varnothing$ \Comment{An empty set.}
\ForAll{$s \in S$}
    \State $Q$.push($s$)
\EndFor
\While{$Q \neq \varnothing$}
    \State $v \gets Q$.pop()
    \State $A$.insert($v$)
    \ForAll{$(u, v) \in E$}
        \If{$u \notin S$}
            \State $Q$.push($u$)
        \EndIf
    \EndFor
\EndWhile
\State \textbf{Result} $A$ \Comment{The result is stored in $A$.}
\end{algorithmic}
\end{algorithm}



==> fig/dataflow-rules-old.tex <==
\newcommand{\stmts}{\mathcal{S}}
\newcommand{\reach}{\mathcal{R}}

\begin{figure}
\begin{prooftree}
    \AxiomC{$e_0 = \text{sandboxed}(\dots,e,\dots) \in \stmts$}
    \AxiomC{$e.\eta \in \mathcal{P}$}
    % \RightLabel{\textcolor{red}{[App]}}
    \BinaryInfC{$e.\eta \in \reach$}
\end{prooftree}


\begin{prooftree}
    \AxiomC{$p_1 = p_2 \in \stmts$}
    \AxiomC{$p_2.\eta \in \reach$}
    % \RightLabel{\textcolor{red}{[App]}}
    \BinaryInfC{$p1.\eta \in \reach$}
\end{prooftree}

\begin{prooftree}
    \AxiomC{$p_1 = \&p_2 \in \stmts$}
    \AxiomC{$p_2.\eta \in \reach$}
    % \RightLabel{\textcolor{red}{[App]}}
    \BinaryInfC{$p1.\eta \in \reach$}
\end{prooftree}   

\begin{prooftree}
    \AxiomC{$p = (*v).\eta_0 \in \stmts$}
    \AxiomC{$v.\eta_0.\eta \in \reach$}
    % \RightLabel{\textcolor{red}{[App]}}
    \BinaryInfC{$p.\eta \in \reach$}
\end{prooftree}   


\begin{prooftree}
    \AxiomC{$(*v).\eta_0 = p \in \stmts$}
    \AxiomC{$p.\eta \in \reach$}
    % \RightLabel{\textcolor{red}{[App]}}
    \BinaryInfC{$v.\eta_0.\eta \in \reach$}
\end{prooftree}   


\begin{prooftree}
    \AxiomC{$ p = \&((*v).\eta_0) \in \stmts$}
    \AxiomC{$v.\eta_0.\eta \in \reach$}
    % \RightLabel{\textcolor{red}{[App]}}
    \BinaryInfC{$p.\eta \in \reach$}
\end{prooftree}   


\begin{prooftree}
    \AxiomC{$ e = f(e_1,e_2,\dots) \in \stmts$}
    % \RightLabel{\textcolor{red}{[App]}}
    \UnaryInfC{$\{e=f.v_0, f.v_1 = e_1, f.v_2 = e_2, \dots\} \subset \stmts$}
\end{prooftree}   

\caption{Rules for computing the backward reachability set $\reach$. } \label{fig:dataflow-rules}
\end{figure}


==> fig/dataflow-rules.tex <==
\newcommand{\stmts}{\mathcal{S}}
\newcommand{\reach}{\mathcal{R}}

\begin{figure}[t]
\begin{algorithmic}[1]
\Require DFG $G = (V, E)$, sandboxed call arguments $\mathit{Args}$
\Ensure Set of cross-boundary allocation sites $\mathit{Allocs}$

\State $\mathit{Worklist} \gets \mathit{Args}$
\State $\mathit{Visited} \gets \emptyset$
\State $\mathit{Allocs} \gets \emptyset$

\While{$\mathit{Worklist} \neq \emptyset$}
    \State $n \gets \mathit{Worklist}.\text{pop}()$
    \If{$n \in \mathit{Visited}$}
        \State \textbf{continue}
    \EndIf
    \State $\mathit{Visited} \gets \mathit{Visited} \cup \{n\}$
    
    \If{$n$ is a heap allocation node}
        \State $\mathit{Allocs} \gets \mathit{Allocs} \cup \{n\}$
    \EndIf
    
    \ForAll{incoming edges $(m, n) \in E$}
        \If{edge is context-compatible}
            \State $\mathit{Worklist}.\text{push}(m)$
        \EndIf
    \EndFor
\EndWhile

\State \Return $\mathit{Allocs}$
\end{algorithmic}
\caption{Backward reachability algorithm for finding cross-boundary heap allocations.
The algorithm traverses the dataflow graph backward from sandboxed call arguments,
collecting all reachable allocation sites.} \label{fig:dataflow-rules}
\end{figure}


==> fig/design-sandbox-runtime.tex <==
\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{fig/asset/design-sandbox-runtime.pdf}
\caption{Sandboxes at runtime.} \label{fig:design-sandbox-runtime}
\end{figure}


==> fig/design-sandbox-syntax.tex <==
\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{fig/asset/design-sandbox-syntax.pdf}
\caption{Sandboxing based on syntax boundaries.} \label{fig:design-sandbox-syntax}
\end{figure}


==> fig/elf-perf.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/svg/elf-rs.png}
    \caption{Running Time of \appname{readelf} Using \libname{elf-rs}.}
    \label{fig:elf-perf}
\end{figure}



==> fig/mir-syntax-old.tex <==
\begin{figure}[t]
\centering

\begin{align*}
\textbf{Type}       & \quad \tau &::=  & \text{bool} \mid \text{i32} \mid \text{Vec}\langle\tau\rangle \mid \&\tau \mid \&\text{mut}\ \tau \mid \dots \\
\textbf{Local}      & \quad v    & \in\ \ & \{ v_0, v_1, v_2, \dots, v_m \} \cup \{v_{m+1}, \dots \} \\
\textbf{Function}   & \quad f    &::=  & \text{f}(v_1, v_2, \dots, v_m) \; \{ s; \} \\
\textbf{Statement}  & \quad s    &::=  & s_1; s_2 \mid e = r \mid e = f(e_1, e_2, \dots) \mid \dots  \\
\textbf{Place}  & \quad e    &::=  & v \mid *e \mid e.\eta \\
\textbf{Rvalue}     & \quad r    &::=  & e \mid \&e \\
\textbf{Projection} & \quad \eta &::=  & \epsilon \mid n.\eta \\
% \textbf{Local Place}      & \quad p    &::=  & v.\eta
\end{align*}
\caption{A simplified grammar of Rust MIR. 
} \label{fig:mir-syntax}
\end{figure}


==> fig/mot-2-spec.tex <==
\begin{figure*}[ht]
\centering
% \begin{lstlisting}[language=Rust]
\begin{minted}[linenos]{toml}
[functions]
handle_request = { syscall = ["read", "write"], transient = true }
\end{minted}
% \end{lstlisting}
\caption{A \toolname{} specification.} \label{fig:mot-2-spec}
\end{figure*}


==> fig/pipeline.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{fig/pdf/annotated-pipeline}
    \caption{\toolname{} compiler pipeline. Components on a darker background indicate additions to conventional \appname{rustc}.}\label{fig:pipeline}
\end{figure*}


==> fig/ripgrep-by-component.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/asset/riggrep-by-component.pdf}
    \caption{Sandboxing \ripgrep{} by components.}
    \label{fig:ripgrep-by-component}
\end{figure}



==> fig/ripgrep-by-file.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/asset/riggrep-by-file.pdf}
    \caption{Sandboxing \ripgrep{} by files.}
    \label{fig:ripgrep-by-file}
\end{figure}



==> fig/servo.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.50\linewidth]{fig/pdf/servo.pdf}
    \caption{Performance overhead of \toolname{} on Servo for different categories in Dromaeo benchmark. \gtan{Not discussed in the main text; consider moving to the appendix.}}
    \label{fig:servo-perf}
\end{figure}



==> fig/snappy-compress.tex <==
\begin{figure}[t]
    \centering
    \includesvg[width=\linewidth]{fig/svg/snappy-compress.svg}
    \caption{Running Time of \libname{snappy} Compression.}
    \label{fig:snappy-compress}
\end{figure}



==> fig/spec-syntax.tex <==
\begin{figure}[t]
\centering

\begin{align*}
\textbf{Spec}       & \quad \Sigma &::=& s^*   \\
\textbf{Section}    & \quad s      &::=& (t\; e)^* \\
\textbf{Title}      & \quad t      &::=& \text{[crates]}  \mid \text{[types]} \mid \text{[functions]}  \\
\textbf{Entity}     & \quad e      &::=& n = \{ \text{transient} = b \}
\end{align*}

\caption{The grammar of \toolname{} specification, where $n$ represents Rust identifiers, $c$ for names of syscalls, and $b$ for a boolean.} \label{fig:spec-syntax}
\end{figure}
% \text{syscall} = [c*], 
% \mid \text{[modules]}


==> fig/transpose-perf.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/svg/transpose.png}
    \caption{Running Time of \appname{RustFFT} Using \libname{transpose}.}
    \label{fig:transpose-perf}
\end{figure}


